Interplay between Federated Learning and Explainable Artificial Intelligence: a Scoping Review

The joint implementation of federated learning (FL) and explainable artificial intelligence (XAI) could allow training models from distributed data and explaining their inner workings while preserving essential aspects of privacy. Toward establishing the benefits and tensions associated with their interplay, this scoping review maps the publications that jointly deal with FL and XAI, focusing on publications that reported an interplay between FL and model interpretability or post-hoc explanations. Out of the 37 studies meeting our criteria, only one explicitly and quantitatively analyzed the influence of FL on model explanations, revealing a significant research gap. The aggregation of interpretability metrics across FL nodes created generalized global insights at the expense of node-specific patterns being diluted. Several studies proposed FL algorithms incorporating explanation methods to safeguard the learning process against defaulting or malicious nodes. Studies using established FL libraries or following reporting guidelines are a minority. More quantitative research and structured, transparent practices are needed to fully understand their mutual impact and under which conditions it happens.

==> archive/latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> archive/old_Section.tex <==

\section{Novel methods combining FL and xAI} \label{s:novel}

We found several research works proposing novel methods, focusing on vertical FL:
\begin{itemize}
    \item In \cite{wang2019interpret}, an explanation scheme is proposed that applies to a binary vertical Federated Learning setting with a host (containing some input features and labels) and a guest (containing a subset of input features different from those contained in the host). The goal is to compute Shapley values for the features contributed by the guest, however due to privacy constraints their values cannot be transferred to the host. The authors solve this situation by clustering all features in the guest into a "united federated feature" that is assigned a Shapley value. The aforementioned Shapley value condenses the contribution to the model output of the guest's features altogether. 
    \item In \cite{chen2022explainableVFL}, an explainable vertical FL method is proposed with:
    \begin{itemize}
        \item Federated counterfactual explanation
        \item Importance rate (IR) metric
    \end{itemize}
    
\end{itemize}

The work in \cite{song2019profit} is specific for Horizontal FL and assigns a Shapley value to each data institution. The aforementioned Shapley value estimates how much the data provided by each institution influences the performance of the model trained via FL. In fact this approach does not provide an explanation in the sense that reveals the model way of predicting, neither it provides the importance of the input features for a specific prediction. However, it provides information about how much information each data center or institution provides to the final model.

Similarly, \cite{wang2020principled} proposes \textcolor{orange}{a principled approach to data valuation for FL}. \acom{TODO: discuss similarities and differences between \cite{song2019profit} and \cite{wang2020principled}}.

\section{Applied work using FL and xAI in combination} \label{s:applied}

A FL scheme is used in \cite{raza2021designing} to train a system that analyzes electrocardiography (ECG) signals for arrythmia classification. The model architecture is based on CNN. After the system is trained via Federated Transfer Learning (FTL) \cite{}, an explanation mechanism based on Grad-CAM \cite{selvaraju2017grad} is applied to highlight the parts of the ECG waveform that are most relevant to the classification output. However, the authors do not assess the possible impact of using a federated training scheme in the quality of the explanations. 

The survey in \cite{saraswat2022explainable} includes a case study that is very similar to the experimental setting in \cite{raza2021designing} \acom{TODO: discuss differences between \cite{saraswat2022explainable} and \cite{raza2021designing} if any}

\subsection{Applied work assessing the impact of FL in explanations} \label{ss:assessing}

Recently, \cite{budig2022} carried out a set of experiments assessing the impact of FL in explanations, becoming (to the best of our knowledge) the first experimental work characterizing FL and xAI in combination. The task in this case is acute stroke patient outcome prediction. Specifically, the authors compare Shapley value summary plots obtained via centralized training vs. those obtained using a federated training scheme. The comparison is done by means of visual inspection of the summary plots and reveals that the FL training produces more scattered and less stable Shapley values than its centralized counterpart. Moreover, the impact of the non-iid data distribution across data centers is evaluated by comparing the results of training with the data distributed across the original data centers with a simulated setting where the data is randomly distributed across a set of "fake" centers. Under this simulated setting, the model's decision boundaries became more complex so it could not provide a clear explanation for an outcome.


\section{Works discussing xAI and FL in practical applications}

\subsection{Networks and Cyber-Security}

In \cite{arisdakessian2022iot}, the authors \textcolor{orange}{
%text marked in orange because these sentences are copied from the original paper and pasted here.
"propose a comprehensive cybersecurity framework that capitalizes on the concepts of XAI, federated learning, game theory and social psychology. We highlight in detail how these concepts can interact all together to provide future IoT systems with strong detection and protection mechanisms against advanced cyberattacks. We argue that such a multidisciplinary cybersecurity framework is needed for future IoT systems in the light of the increasingly complex and elaborate cyberattacks that are being constantly crafted. When discussing the future directions in the field, they propose a multi-disciplinary cybersecurity framework that combines the concepts of XAI, federated learning, game theory and social psychology to provide strong detection and protection solutions to future IoT systems."} \acom{unfortunately we will probably exclude this paper as it discusses FL and xAI separately and the discussion on xAI is too shallow}

In \cite{torre2022interpretable}, the authors \textcolor{orange}{
\begin{itemize}
    \item develop a transformer-based learning system to detect cyber-security threats from text-based system logs. The transformer is trained in a federated setting to preserve the sensitive information contained in the logs at each individual server, and an interpretability module is implemented to provide forensic investigators the means to backtrack the log keys triggering a cyber-threat detection. 
    \item The transformer is trained using FedAvg~\cite{mcmahan2017communication} following a typical horizontal FL architecture and, after the last federated iteration, the interpretability module at each client computes the interpretability weights using the latest global FL model. Clients then share the weights with the FL server who aggregates them to generate the federated interpretability weights.
    \item The input data is a stream of log messages that is converted into a time-series of log keys by means of a log parser. The transformer is trained to predict which log keys are most likely to come next, and this prediction is compared against the ground-truth key to detect anomalous patterns, which are identified as possible cyber attacks.
    \item In order to backtrace the source of detected anomalies, the interpretability module presents the sequence of log keys that triggered the detection of an anomaly and the attention for each key in the input sequence. If a log key is classified as abnormal, the sequence of log keys that initiated the incident can be tracked down.
    \item The predictor architecture is a transformer-based model with multi-head attention.
    \item The interpretability module at each client provides insight to the level of influence each unique log key has in a particular sequence of log keys. The federated transformer log learning model is used by the interpretability module to evaluate a given sequence S.
    \item At each iteration, a set of so-called interpretability weights are calculated, which aggregate the attention associated with each log key. Each client sends the interpretability weights to the FL server, which in turn aggregates the computed weights from each client and afterwards shares the federated interpretability weights with each client. 
    \item The attention mechanism learns how much importance to assign to each log key to predict a subsequent log key. Attention weights represent the memory acquired while learning the relationship between log keys in the input sequence and corresponding predictions. The attention-based interpretability module aggregates attention calculated in the transformed model, and is used to generate a visualization of the attention distribution, which is expected to be different from normal operations when a cyber-threat is present.
\end{itemize}
}

\subsection{Biomedical applications}

\acom{list here all papers in the survey that apply FL and xAI in the medical domain}.

==> archive/old_abstract.tex <==
Federated learning (FL) allows training models from distributed data while preserving important aspects of privacy. Explainable artificial intelligence (XAI) aims to explain the inner workings of machine learning (ML) algorithms, thereby increasing transparency. The joint implementation of FL and XAI is expected to provide both benefits, but their interplay could create tensions %and tradeoffs
between comprehension and privacy. While extensive research has addressed these two technologies, it is not established whether they are in conflict, can be addressed separately, or what the potential interactions are. To answer this question, this scoping review maps those publications that jointly deal with FL and XAI, either from a methodological or experimental perspective.%, and the reported kinds of interplay. 
We specifically focused on publications where an interplay between FL and model interpretability or post-hoc explanations was found. %For XAI, both model interpretability and post-hoc explanation methods were considered. 
%We analyzed how the authors jointly deal with FL and XAI and the reported kinds of interplay. 

The diverse XAI methods and FL setups are charted together with the nature and amount of data used in each study. In total, 37 studies met the criteria, with more papers focusing on explanation than on interpretability methods.
Feature relevance was the predominant type of explanation, whereas algorithmic transparency was the most common type of model interpretability. The predominant type of FL was horizontal, most works used simulated FL setups and involved less than 10 data centers.
%Most of the relevant studies were applied in medicine/life sciences and finance. Studies reported influence of FL on XAI only upon experimenting with more than 1,000 data points.

We found only one study that explicitly and quantitatively analyzed the influence of FL on model explanations, revealing an interesting and significant research gap. In several reviewed cases, aggregation of interpretability metrics across FL nodes created generalized global insights at the cost of some degree of local interpretability. For instance, studies showed that while global models achieved broader generalizability, individual patterns unique to each node were often diluted. Incorporating explanation methods as a component of the FL algorithm design seems like a promising avenue, since 8 reviewed papers reported on the benefits of such practice.

Studies using established FL libraries or following reporting guidelines are still a minority. This review underscores the need for more structured and transparent research practices in the intersection of FL and XAI, in addition to more studies quantifying the impact of one on the other, to determine their mutual impact and under which conditions it happens.

==> figures/pie-chart-data-types.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{tikz/pie-chart-data-types}
    \caption{Distribution of reviewed papers across the different types of data used in their experiments. Clinical and finance data are predominant.}\label{fig:type_of_data}
\end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{images/type_of_data.png}
%     \caption{Distribution of reviewed papers across the different types of data used in their experiments. Clinical and finance data are predominant.}%Adam
%     \label{fig:type_of_data}
% \end{figure}

